How to Bridge the Gap between Modalities: Survey on Multimodal Large Language Model

We explore Multimodal Large Language Models (MLLMs), which integrate LLMs like GPT-4 to handle multimodal data, including text, images, audio, and more. MLLMs demonstrate capabilities such as generating image captions and answering image-based questions, bridging the gap towards real-world human-computer interactions and hinting at a potential pathway to artificial general intelligence. However, MLLMs still face challenges in addressing the semantic gap in multimodal data, which may lead to erroneous outputs, posing potential risks to society. Selecting the appropriate modality alignment method is crucial, as improper methods might require more parameters without significant performance improvements. This paper aims to explore modality alignment methods for LLMs and their current capabilities. Implementing effective modality alignment can help LLMs address environmental issues and enhance accessibility. The study surveys existing modality alignment methods for MLLMs, categorizing them into four groups: (1) Multimodal Converter, which transforms data into a format that LLMs can understand; (2) Multimodal Perceiver, which improves how LLMs percieve different types of data; (3) Tool Learning, which leverages external tools to convert data into a common format, usually text; and (4) Data-Driven Method, which teaches LLMs to understand specific data types within datasets.

==> utils/mllms.tex <==
\begin{table*}[!h]
    \centering
      \caption{
        The Statistics of Multimodal Large Language Models(MLLMs). 
        \textbf{Release Time} is the first version's time as listed on arXiv. 
        \textbf{First Affiliation} indicates the primary affiliation of the first author in the paper. 
        \textbf{Backbone LLM} signifies the foundational large model used for experimentation in the MLLM.
        \textbf{Multimodal encoder} details the method employed by the MLLM to perceive specific modal information. 
        \textbf{Alignment pattern} is a categorization based on various methods outlined in our paper, such as `1-DirectMapping' representing the first alignment method summarized in the 'Direct Mapping' mode within the '1Multimodal Converter.' 
        \textbf{Support Modalities} outlines the formats of input information supported by this model, including images, text, videos, and more. 
        \textbf{Training Pattern} encompasses the training methods mentioned in the model's paper, involving training solely the intermediate part of modality linking (linear layer), single-stage instruction tuning, and two-stage pre-training followed by instruction tuning. 
        Lastly, \textbf{Publication} documents the platforms where these models were published up until the submission of our paper.
    }
    \resizebox{0.95\textwidth}{!}
    { 
    \begin{tabular}{llccccccc}
    \toprule
        \textbf{MLLM} & \textbf{Release time} & \textbf{First affiliation} & \textbf{Backbone LLM} & \textbf{Multi-modal encoder} & \textbf{Alignment pattern} & \textbf{Supported modalities} & \textbf{Training pattern} & \textbf{Publication} \\
        \hline
        PICa~\cite{PICa} & 10-Sep-21 & Microsoft & GPT3 & VinVL-base & 1-Textual Conversion & Text, Image & One stage trainig & AAAI22 \\
        \hline
        KAT~\cite{KAT} & 16-Dec-21 & \makecell{Carnegie Mellon\\ University} & T5 & CLIP(ViT-B/16) & 1-Textual Conversion & Text, Image & One stage trainig & NAACL22\\
        \hline
        SMs~\cite{SMs} & 01-Apr-22 & Google  & - & CLIP & \makecell{3-Natural language\\ assisted-coordinators} & Text, Image, Audio & One stage reasoning & ICLR23\\
        \hline
        Flamingo~\cite{Flamingo}  & 29-Apr-22 & Deepmind  & Transformer &\makecell{ Visual Encoder Pretrained \\on the ALIGN and LTIP} & 2-Customization
        Perceiver & Text, Image & Two stage training & NeurIPS22\\
        \hline
         GIT~\cite{Git}& 27-May-22& Microsoft& -& Swin-like vision transformer& 1-Direct Mapping& Text, Image, Video&Two stage training& TMLR23\\
        \hline
         REVIVE~\cite{REVIVE}&02-Jun-22& \makecell{University of \\Washington}& T5& CLIP(ViT-B/16)& 1-Textual Conversion& Text, Image& One stage traning& NeurIPS22  \\
        \hline
         VISPROG~\cite{VISPROG} & 18-Nov-22 & Allen Institute for AI & GPT3 & Tools: Stable Diffusion, MaskFormer & 3-Natural & Text, Image, & One stage reasoning & CVPR23 \\
        \hline
         BLIP-2~\cite{blip2} & 30-Jan-23 & Salesforce Research & OPT2.7B/6.7B, FlanT5 & CLIP(ViT-L/14), EVA-CLIP(ViT-g/14) & 2-Q-Former & Text, Image & One stage pretraining & ICML23 \\
        \hline
        FROMAGe~\cite{FROMAGe} & 31-Jan-23 & \makecell{Carnegie Mellon\\ University} & OPT & CLIP ViT-L/14 & 1-Direct Mapping & Text, Image & \makecell{Connection module\\ training} & ICML23 \\
        \hline
        ML-MFSL~\cite{ML_MFSL} & 28-Feb-23 & \makecell{University of \\Amsterdam} & GPT2 & CLIP & 1-Direct Mapping & Text, Image &  \makecell{Connection module\\ training} & NeurIPS22 \\
        \hline
        Prophet~\cite{prophet} & 03-Mar-23 & \makecell{Hangzhou Dianzi\\ University} & GPT3 & CLIP & 1-Adapter-based & Text, Image & One stage traning & CVPR23 \\
        \hline
        ViperGPT~\cite{ViperGPT} & 14-Mar-23 & Columbia University & ChatGPT & \makecell{Tools:GLIP, MiDaS,\\ BLIP-2, X-VLM, GPT3\\ for llm-query, Codex} & 3-Natural & Text, Image, Code & One stage reasoning & arXiv \\
        \hline
        MM-REACT~\cite{MM-REACT} & 20-Mar-23 & Microsoft Azure AI & ChatGPT & Azure Cognitive Services APIs & 3-Natural & Text, Image & One stage reasoning & arXiv \\
        \hline
         LLaMA-Adapter~\cite{llama_adpater} & 28-Mar-23 & Shanghai AI Lab & Llama & ViT & 1-Adapter-based & Text, Image & One stage traning & arXiv \\
        \hline
        TaskMatrix.AI~\cite{TaskMatrix.AI} & 29-Mar-23 & Microsoft & Millions of APIs & Tools: Millions of APIs & 3-Natural & \makecell{Text, Image, Video,\\ Audio, Music, Location} & One stage reasoning & arXiv \\
        \hline
        HuggingGPT~\cite{HuggingGPT} & 30-Mar-23 & Zhejiang University & ChatGPT3.5/4 & Tools: yolos-tiny /detr-resnet-101. & 3-Natural & Text, Image, Pose & One stage reasoning & arXiv \\
        \hline
        ChatCaptioner~\cite{ChatCaptioner} & 09-Apr-23 & \makecell{King Abdullah University of\\ Science and Technology} & ChatGPT and BLIP-2 & Included in based-LLM & 3-Natural & Text, Image, Video, Audio & One stage reasoning & arXiv \\
        \hline
         Llava~\cite{llava} & 17-Apr-23 & \makecell{University of \\Wisconsin–Madison} & Vicuna & CLIP ViT-L/14 & 1-Direct Mapping & Text, Image & Two stage training & arXiv \\
        \hline
        CancerGPT~\cite{CancerGPT}    & 18-Apr-23 & \makecell{School of Information University\\ of Texas at Austin}  & GPT2 & Not Mentioned & 4-Disciplinary expertise & Text, BioMedicine Image & One stage reasoning & arXiv\\
        \hline
        Chameleon~\cite{Chameleon} & 19-Apr-23 & \makecell{University of California,\\ Los Angeles} & GPT-4 & \makecell{Tools: Bing Search API,\\ Python Program Verifier} & 3-Natural & Text, Image, Code & One stage reasoning & NeruIPS23 \\
        \hline
        MiniGPT4~\cite{Minigpt-4} & 20-Apr-23 & \makecell{King Abdullah University of\\ Science and Technology} & Llama2, Vicuna-13B/7B & EVA-CLIP(ViT-g/14) & 2-Q-Former & Text, Image & Two stage training & arXiv \\
        \hline
        LLaMA-Adapter2~\cite{llama_adpterv2} & 28-Apr-23 & Shanghai AI Lab & Llama & CLIP; BLIP, DocVQA & 1-Adapter-based & Text, Image & One stage traning & arXiv \\
        \hline
        23CAT~\cite{CAT} & 04-May-23 & SUSTech VIP Lab & ChatGPT & Tools: SAM, BLIP2, ChatGPT API & 3-Natural & \makecell{Text, Image,\\ Points, Boxes, Trajectory} & One stage reasoning& arXiv \\
        \hline
        Otter~\cite{otter} & 05-May-23 & \makecell{Nanyang Technological\\ University} & OpenFlamingo & Included in based-LLM & 2-Customization & Text, Image &\makecell{One stage instruction\\ tuning }& arXiv \\
        \hline
        MultiModal-GPT~\cite{MultiModal-GPT} & 08-May-23 & Shanghai AI Lab & Llama7B, OpenFlamingo & CLIP & \makecell{2-Customization, \\4-Instruction-following}  & Text, Image & \makecell{One stage instruction\\ tuning }& arXiv \\
        \hline
        VideoChat~\cite{Videochat} & 10-May-23 & Shanghai AI Lab & BLIP2, StableVicuna & ViT-G & 1-Direct Mapping & Text, Video & Two stage traning & arXiv \\
        \hline
        VisionLLM~\cite{visionllm} & 18-May-23 & Shanghai AI Lab & Alpaca-7B & ResNet and InternImage-H & 2-Customization & Text, Image & One stage reasoning & NeruIPS23 \\
        \hline
        VideoLLM~\cite{VideoLLM} & 22-May-23 & Nanjing University & GPT2, T5, OPT & \makecell{LSTR,Testra, ASFormer, \\SS-TCN, MS-TCN, Ego4D, \\VSGN, InternVideo, Moment DETR} & 1-Direct Mapping & Text, Image, Video & \makecell{One stage instruction\\ tuning }& CVPR23 \\
        \hline
        IdealGPT~\cite{IdealGPT} & 24-May-23 & Columbia University & ChatGPT & Not Mention & 3-Natural & Text, Image & One stage reasoning& ACL23 \\
        \hline
        PandaGPT~\cite{PandaGPT} & 25-May-23 & University of Cambridge & Vicuna & ImageBind & 2-Customization & \makecell{Text, Image, Video, Audio,\\ depth, thermal, and\\ inertial measurement units (IMU)} & \makecell{One stage instruction\\ tuning }& ACL23 \\
        \hline
        LLaVA-Med~\cite{Llava-med} & 01-Jun-23 & Microsoft & Vicuna & BioMedCLIP & 4-Disciplinary expertise & Text, BioMedicine Image & \makecell{Two stage alignment \\and instuction tuning} & NeruIPS23 \\
        \hline
        Video-LLaMA~\cite{Video-llama} & 05-Jun-23 & \makecell{DAMO Academy, \\Alibaba Group} & Vicuna, Llama & ViT, ImageBind & 2-Q-Former & Text, Image, Video, Audio & Two stage training & EMNLP23 \\
        \hline
        LAMM~\cite{lamm} & 11-Jun-23 & Shanghai AI Lab & Vicuna-13B & CLIP(ViT-L/14); FrozenCLIP & 4-Complex modalities & Text, Point Cloud & \makecell{Connection module\\ training} & NeruIPS23 \\
        \hline
        AVIS~\cite{AVIS} & 13-Jun-23 & \makecell{University of California,\\ Los Angeles} & PALM 540B & \makecell{Tools: PALI, Google Lens,\\ Google Web Search API} & 3-Natural & Text, Image & One stage reasoning & NeruIPS23 \\
        \hline
        AssistGPT~\cite{AssistGPT}& 14-Jun-23 & \makecell{National University\\ of Singapore} & FlanT5, Vicuna7B  &  \makecell{Tools:BLIP2, Google OCR,\\ OpenAI’s open-source ASR,\\ assisted-Code etc.} & 3-Both assisted & Text, Image, Video, Code & One stage reasoning & arXiv \\
        \hline
        MACAW~\cite{Macaw-LLM} & 15-Jun-23 & Tencent AI Lab & Llama-7b & CLIP, WHISPER for Audio, & 2-Customization & Text, Image, Video, Audio & \makecell{One stage instruction\\ tuning }& arXiv \\
        \hline
        GAVIE~\cite{GAVIE} & 26-Jun-23 & University of Maryland & MiniGPT4/mPLUG-Owl & ViT & 2-Q-Former & Text, Image & \makecell{One stage instruction\\ tuning }& arXiv \\
        \hline
        Shikra~\cite{shikra} & 27-Jun-23 & SenseTime Research & Vicuna-7/13B & CLIP(ViT-L/14) & 4-Spatial comprehension & Referential Dialogue, Image & \makecell{One stage instruction\\ tuning }& arXiv \\
        \hline
        LENS~\cite{LENS} & 28-Jun-23 & Contextual AI & Flan-T5 & OpenCLIP-H/14, CLIP-L/14, BLIP & 1-Textual Conversion & Text, Image & Two stage training & arXiv \\
        \hline
        LLaVAR~\cite{LLaVAR} & 29-Jun-23 & Georgia Tech & Vicuna-13B & \makecell{CLIP-ViT-L/14, CLIP-ViT-L/14-336} & 4-Instruction-following & Text, Image & \makecell{One stage instruction\\ tuning }& arXiv \\
        \hline
        SPAE~\cite{SPAE} & 30-Jun-23 & Google Research & GPT 3.5 / PaLM 2 & CLIP(ViT-L/14) & 2-VAE Perceive & Text, Image & One stage reasoning & NeruIPS23 \\
        \hline
        Lynx~\cite{Lynx} & 05-Jul-23 & ByteDance Research & LLaMA-7B/ Vicuna-7B & EVA-1B & 1-Direct Mapping & Text, Image, Video & Two stage training & arXiv \\
        \hline
         GPT4ROI~\cite{GPT4ROI} & 07-Jul-23 & \makecell{The University of\\ Hong Kong} & Llama7B & CLIP & 4-Spatial comprehension &Text, Image & Two stage training & arXiv \\
        \hline
        VoxPoser~\cite{Voxposer} & 12-Jul-23 & Stanford University & GPT-4 & OWL-ViT, XMEM & 1-Adapter-based & Text, Image, Video & One stage Instuction Tuning & arXiv \\
        \hline
        OpenFlamingo~\cite{OpenFlamingo} & 02-Aug-23 & University of Washington & MPT, RedPajama & CLIP ViT-L/14 & 2-Customization & Text, Image & \makecell{One stage instruction\\ tuning }& arXiv \\
        \hline
        VPG-C~\cite{VPG-C} & 08-Aug-23 & Zhejiang University & Vicuna-7B, Llama2-7B & EVA-CLIP(ViT-g/14) & 2-Q-Former & Text, Image & One stage FineTuning & arXiv \\
        \hline
        BLIVA~\cite{BLIVA} & 19-Aug-23 & UC San Diego & Vicuna-7B & EVA-CLIP(ViT-g/14) & 2-Q-Former & Text, Image, Video & Two stage training & AAAI24 \\
        \hline
        PointLLM~\cite{pointllm}&31-Aug-23 &\makecell{The Chinese University\\ of Hong Kong} &Vicuna7B, Vicuna 13B & Point-BERT &4-Complex modalities &Text, Point clouds image & One stage Instuction Tuning & arXiv\\
        \hline
        NExT-GPT~\cite{NExT-GPT} & 11-Sep-23 & \makecell{National University\\ of Singapore} & Vicuna & ImageBind & 1-Direct Mapping & Text, Image, Video, Audio & \makecell{Connection module\\ training} & arXiv \\
        \hline
        MMICL~\cite{MMICL} & 14-Sep-23 & Peking University & FLANT5-XL/XXL & EVA-CLIP(ViT-g/14) & 2-Q-Former & Text, Image & Two stage training & arXiv \\
        \hline
        DREAMLLM~\cite{DreamLLM} & 20-Sep-23 & \makecell{Xi’an Jiaotong\\ University} & Vicuna & CLIP-Large+Stable Diffusion & 1-Direct Mapping & Text, Image & \makecell{Three stage training: \\Alignment Training, \\L-GPT Pretraining, \\Supervised Fine-tuning} & arXiv \\
          \hline
          InternLM-\cite{InternLM-XComposer} & 26-Sep-23 & Shanghai AI Lab & InternLM & EVA-CLIP(ViT-g/14) & 2-Q-Former & Text, Image & Two stage training & arXiv \\
        \hline
         MiniGPT5~\cite{MiniGPT-5} &	03-Oct-23 & \makecell{University of California,\\ Santa Cruz} & Llama2, Vicuna-13B/7B & ViT&2-Q-Former &Text, Image & Two stage training& arXiv\\
        \hline
        OtterHD~\cite{OtterHD} & 07-Nov-23& \makecell{Nanyang Technological\\ University} & Fuyu-8B & ViT & 4-Instruction-following & Text, Image &  One stage Instuction Tuning & arXiv \\
        \hline
        ShareGPT4V~\cite{ShareGPT4V} &21-Nov-23 & \makecell{University of Science\\ and Technology of China} &Vicuna7B, Vicuna13B	& GPT4-vision & 4-Enhanced image comprehension & Text, Image & Two stage training & arXiv\\
        \bottomrule
    \end{tabular}
    }
    \label{tab:Statistics}
\end{table*}
